Interrupting Real-Time IoT Tasks: How Bad Can It Be to Connect Your Critical Embedded System to the Internet?

Embedded systems have been used to control physical environments for decades. Usually, such use cases require low latencies between commands and actions as well as a high predictability of the expected worst-case delay. To achieve this on small, low-powered microcontrollers, Real-Time Operating Systems (RTOSs) are used to manage the different tasks on these machines as deterministically as possible. However, with the advent of the Internet of Things (IoT) in industrial applications, the same embedded systems are now equipped with networking capabilities, possibly endangering critical real-time systems through an open gate to interrupts. This paper presents our initial study of the impact network connections can have on real-time embedded systems. Specifically, we look at three aspects: The impact of network-generated interrupts, the overhead of the related networking tasks, and the feasibility of sharing computing resources between networking and real-time tasks. We conducted experiments on two setups: One treating NICs and drivers as black boxes and one simulating network interrupts on the machines. The preliminary results show that a critical task performance loss of up to 6.67% per received packet per second could be induced where lateness impacts of 1% per packet per second can be attributed exclusively to ISR-generated delays.

==> inc/2_background.tex <==
\section{Background}
\label{sec:background}
Wi-Fi networking introduces a number of tasks for connection, maintenance and packet handling. This section will give a short introduction into the management of Wi-Fi connections and the path of a received network packet through a microcontroller.

\subsection{Packet Handling}
Packets work their way up the network stack beginning in the physical layer arriving at the \gls{nic}. The payload of the data frame is received into a packet queue using Direct Memory Access (DMA), and that memory area is mapped directly into the kernel space of the operating system. At this point, the processor is notified of the arrival of a new packet by an interrupt triggered through the driver.

General computing kernels like Linux transfer computational intensive packet processing work from the hardware triggered interrupts into \textit{softirqs} (tasklets) that are scheduled and run with the second highest priority in the system \cite{irqlinux}. On the other hand, embedded network device drivers are often shipped together with the network stack and offer a network interface abstraction. The network stack registers receive and transmit callbacks to the network driver which then are invoked upon packet reception and transmission. an example process flow can be seen in Figure \ref{fig:background}.

\begin{figure}[hb]
\centering
\includegraphics[scale=1]{img/background.pdf}
\caption{Process flow for received IP packets in \glspl{mcu}.}
\label{fig:background}
\end{figure}

\subsection{Stack Overview (LwIP)}
The different network stack implementations vary in their set of features. The \textsc{lw}IP network stack is widely spread among embedded applications and sets its focus on memory efficiency \cite{lwip}. It covers the majority of commonly used and necessary protocols from Layer 2 up to Layer 4 like ARP, IP, TCP, UDP, DNS, and DHCP. It offers different APIs for efficient access, multi-threading, and an implementation of the Berkley Socket API. Internally, \textsc{lw}IP does not represent a complete data frame but stores a subset of data in \texttt{pbuf} structures. Other stack implementations like FreeRTOS+TCP offer the complete frame and stick to the Berkeley sockets API while being thread-safe.

%\subsection{Application}
%Embedded devices with networking capabilities find their usage in IoT applications from cars, home automation, health monitoring, smart farming or different wireless sensor networks and production processes in industry 4.0. The role of embedded devices in IoT is to connect sensors to a bigger network whose backends generate real-time reactions based on the given sensor data. These calculated actions are then executed by embedded devices which in turn control (physical) actuators.

%Since interrupts to embedded devices' processing cores are naturally unpredictable, and their occurences in a closed system or small isolated network are low and in a controllable frame, connecting these microprocessors with usually tiny amount of processing power to the internet might expose critical infrastructure to the dangers of the internet including high traffic, DoS or DDoS attacks.

